RGB-D Object Detection and Semantic Segmentation for Autonomous Manipulation in Clutter

Autonomous robotic manipulation in clutter is challenging. A large variety of objects must be perceived in complex scenes, where they are partially occluded and embedded among many distractors, often in restricted spaces. To tackle these challenges, we developed a deep-learning approach that combines object detection and semantic segmentation. The manipulation scenes are captured with RGB-D cameras, for which we developed a depth fusion method. Employing pretrained features makes learning from small annotated robotic data sets possible. We evaluate our approach on two challenging data sets: one captured for the Amazon Picking Challenge 2016, where our team NimbRo came in second in the Stowing and third in the Picking task, and one captured in disaster-response scenarios. The experiments show that object detection and semantic segmentation complement each other and can be combined to yield reliable object perception.

==> results/apc_design_choices.tex <==
\pgfplotstableread{results/apc_results.txt}\apcresults
\begin{threeparttable}
 \caption[Object detection architectures]{%
   Evaluation of object detection architectures on the shelf dataset.
   The mAP object detection score and the F1 localization score are shown for each architecture.
 }
 \label{tab:apc:architectures}
 \pgfplotstabletypeset[
  highlight col max={\apcresults}{informed_mAP},
  highlight col max={\apcresults}{uninformed_mAP},
  highlight col max={\apcresults}{F1},
  columns/{Dataset}/.style={string type,
    column name={Input},
    column type=l,
    string replace={depth-hhav}{RGB-D (TGV)},
    string replace={depth-upper-hhav}{RGB-D (single)\tnote{1}},
    string replace={merged}{RGB},
    string replace={depth-old}{RGB-D (DT)\tnote{2}},
  },
  columns/{Variant}/.style={string type,
    column type=l,
    string replace={notailor}{SVM (plain)},
    string replace={tailor}{SVM (tailor)},
    string replace={hha_concat}{HHA Features (Fig.~\ref{fig:method:depth:downsample})}, %  (Sec.~\ref{sec:method:depth:hha_concat})
    string replace={hha_cnn}{HHA CNN (Fig.~\ref{fig:method:depth:2cnn})}, %  (Sec.~\ref{sec:method:depth:hha_cnn})
    string replace={normal}{Softmax (with augmentation)},
    string replace={noaug}{Softmax (no augmentation)},
    string replace={cross}{Distillation}, %  (Sec.~\ref{sec:method:depth:distillation})
    string replace={proposal}{Ext. Proposals}, %  (Sec.~\ref{sec:method:depth:proposals})
  },
  columns/{uninformed_mAP}/.style={
    column name={Uninf.},
    zero to dash,
    fixed zerofill,
    multiply with=0.01,
    precision=3,
  },
  columns/{informed_mAP}/.style={
    column name={Inf.},
    fixed zerofill,
    multiply with=0.01,
    precision=3,
  },
  columns/{F1}/.style={
    fixed zerofill,
    multiply with=0.01,
    precision=3,
  },
  every head row/.style={
    before row={
      \toprule
       & & \multicolumn{2}{c}{mAP} \\
       \cmidrule(r){3-4}
    },
    after row=\midrule
  },
  every last row/.style={after row=\bottomrule},
  every row no 1/.style={after row=\midrule},
  every row no 3/.style={after row=\midrule},
  every row no 7/.style={after row=\midrule},
 ]{\apcresults}
 \begin{tablenotes}
  \item[1] Without depth fusion, only from upper camera. Filled using TGV method.
  \item[2] Old filling method used during APC 2016 based on a color-guided smoothing filter.
 \end{tablenotes}
 \end{threeparttable}
 
